C2HLSC: Can LLMs Bridge the Software-to-Hardware Design Gap?

High Level Synthesis (HLS) tools offer rapid hardware design from C code, but their compatibility is limited by code constructs. This paper investigates Large Language Models (LLMs) for refactoring C code into HLS-compatible formats. We present several case studies by using an LLM to rewrite C code for NIST 800-22 randomness tests, a QuickSort algorithm and AES-128 into HLS-synthesizable c. The LLM iteratively transforms the C code guided by user prompts, implementing functions like streaming data and hardware-specific signals. This evaluation demonstrates the LLM's potential to assist hardware design refactoring regular C code into HLS synthesizable C code.

==> waves.tex <==
\begin{figure}[!tb]
  \centering
  \includegraphics[width=\columnwidth]{images/monobit.png}
  \vspace*{-20pt}
  \caption{Monobit waveform.}
  \vspace*{-20pt}
  \label{fig:wave}  % Optional label for referencing
  
\end{figure}

\begin{figure}[!tb]
  \centering
  \includegraphics[width=\columnwidth]{images/block.png}
  \vspace*{-20pt}
  \caption{Monobit Block waveform.}
  \vspace*{-20pt}
  \label{fig:wave}  % Optional label for referencing
  
\end{figure}

\begin{figure}[!tb]
  \centering
  \includegraphics[width=\columnwidth]{images/cusums.png}
  \vspace*{-20pt}
  \caption{Cumulative Sums waveform.}
  \vspace*{-20pt}
  \label{fig:wave}  % Optional label for referencing
  
\end{figure}

\begin{figure}[!tb]
  \centering
  \includegraphics[width=\columnwidth]{images/overlapping.png}
  \vspace*{-20pt}
  \caption{Overlapping Template Matching waveform.}
  \vspace*{-20pt}
  \label{fig:wave}  % Optional label for referencing
  
\end{figure}
